A Simple and Strong Baseline for End-to-End Neural RST-style Discourse Parsing

To promote and further develop RST-style discourse parsing models, we need a strong baseline that can be regarded as a reference for reporting reliable experimental results. This paper explores a strong baseline by integrating existing simple parsing strategies, top-down and bottom-up, with various transformer-based pre-trained language models. The experimental results obtained from two benchmark datasets demonstrate that the parsing performance strongly relies on the pretrained language models rather than the parsing strategies. In particular, the bottom-up parser achieves large performance gains compared to the current best parser when employing DeBERTa. We further reveal that language models with a span-masking scheme especially boost the parsing performance through our analysis within intra- and multi-sentential parsing, and nuclearity prediction.

==> contents/tables/ablation.tex <==
\renewcommand{\arraystretch}{0.9}
\begin{table}[tb]
    \centering
    \setlength{\tabcolsep}{2pt}
    \small
    \begin{tabular}{lcccc}
    \toprule
      & \multicolumn{2}{c}{\textbf{RST-DT}} & \multicolumn{2}{c}{\textbf{Instr-DT}}\\
      \cmidrule(lr){2-3}\cmidrule(lr){4-5}
     & \textbf{Dev.} & \textbf{Test} & \textbf{Dev.} & \textbf{Test}\\
        \midrule
        Top-down      & 56.3~(0.10) & 55.1~(0.12) & 49.1~(0.81) & 41.9~(0.32)\\
        ~~-org. feat. & 55.9~(0.09) & 54.4~(0.23) & 48.4~(0.24) & 43.4~(0.26)\\
        \midrule
        Bottom-up     & 56.1~(0.58) & 55.2~(0.49) & 51.0~(1.28) & 43.3~(1.32)\\
        ~~-org. feat. & 55.6~(0.29) & 54.4~(0.50) & 50.3~(0.27) & 44.4~(1.20)\\
        \bottomrule
    \end{tabular}
    \caption{Fully labeled span F1 scores w/ and w/o organization features (with DeBERTa).}% \texttt{base}).}
     \label{tab:ablation}
    \end{table}

==> contents/tables/dep_instrdtLi14.tex <==
\renewcommand{\arraystretch}{0.85}
\begin{table*}[t]
    \centering
    \small
    %\begin{tabular}{llPPPPPP}
    \begin{tabular}{llcccccc}
    \toprule
     & \multirow{2}{*}{} & \multicolumn{3}{c}{\textbf{UAS}} & \multicolumn{3}{c}{\textbf{LAS}}\\       
    \cmidrule(lr){3-5}\cmidrule(lr){6-8}
    & & \textbf{All}~$\boldsymbol{(d=*)}$ & $\boldsymbol{d=0}$ & $\boldsymbol{d \ge 1}$ & \textbf{All}~$\boldsymbol{(d=*)}$ & $\boldsymbol{d=0}$ & $\boldsymbol{d \ge 1}$ \\
        \midrule
    \multirow{5}{*}{\rotatebox[origin=c]{90}{Top-down}}
            & BERT     & 62.8~(0.71) & 78.7~(0.35) & 32.9~(1.82) & 43.6~(0.44) & 55.2~(0.35) & 19.0~(1.19)\\
            & RoBERTa  & \textbf{67.9}~(0.60) & \textbf{82.3}~(0.58) & 41.2~(0.95) & \textbf{49.5}~(0.61) & \textbf{59.9}~(0.20) & 27.4~(1.56)\\
            & XLNet    & 66.6~(0.32) & 80.0~(0.47) & 41.2~(0.95) & 48.3~(0.30) & 58.7~(0.53) & 26.2~(0.69)\\
            & SpanBERT & 66.3~(1.96) & 80.4~(1.41) & 39.8~(3.12) & 46.0~(3.15) & 56.6~(3.32) & 23.2~(3.69)\\
            & DeBERTa  & 67.6~(1.68) & 79.6~(2.02) & \textbf{44.5}~(1.44) & \textbf{49.5}~(1.24) & 58.3~(1.88) & \textbf{30.1}~(1.34)\\
        \midrule
       \multirow{5}{*}{\rotatebox[origin=c]{90}{Bottom-up}} 
            & BERT     & 62.9~(1.51) & 79.9~(2.16) & 31.3~(0.76) & 42.6~(1.62) & 54.4~(1.96) & 17.5~(1.25)\\
            & RoBERTa  & 66.6~(1.23) & 80.8~(1.11) & 39.9~(2.13) & 49.7~(1.53) & 60.6~(0.82) & 26.7~(3.15)\\
            & XLNet    & \textbf{71.0}~(1.10) & 84.1~(0.47) & \textbf{46.6}~(2.82) & 51.9~(1.04) & 61.5~(0.91) & \textbf{31.3}~(2.13)\\
            & SpanBERT & 66.3~(0.79) & 79.4~(0.77) & 41.4~(1.01) & 48.3~(0.60) & 58.8~(1.38) & 25.9~(0.87)\\
            & DeBERTa  & 70.3~(0.75) & \textbf{84.2}~(0.42) & 44.4~(2.69) & \textbf{52.0}~(0.89) & \textbf{61.8}~(1.17) & 31.0~(3.97)\\
        \bottomrule
    \end{tabular}
    \caption{Results in dependency format obtained from Instr-DT.}
     \label{tab:result_dep_instr_Li14}
    \end{table*}


==> contents/tables/dep_rstdt.tex <==
\renewcommand{\arraystretch}{0.9}
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{llPPPPPP}
    \toprule
     & \multirow{2}{*}{} & \multicolumn{3}{c}{\textbf{UAS}} & \multicolumn{3}{c}{\textbf{LAS}}\\       
    \cmidrule(lr){3-5}\cmidrule(lr){6-8}
    & & \textbf{All} & $\boldsymbol{d=1}$ & $\boldsymbol{d>1}$ & \textbf{All} & $\boldsymbol{d=1}$ & $\boldsymbol{d>1}$ \\
        \midrule
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Top-down}}
            & BERT     & 61.7~(1.01) & 83.6~(0.95) & 41.2~(1.15) & 48.0~(1.21) & 70.1(0.88) & 27.1~(1.60)\\
            & SpanBERT & 64.8~(0.23) & 86.3~(0.78) & 44.9~(1.14) & 51.9~(0.22) & 74.2(0.83) & 30.9~(1.19)\\
            & RoBERTa  & 67.1~(0.32) & 88.3~(0.42) & 47.5~(0.81) & 52.6~(0.67) & 75.8~(0.37) & 30.9~(1.07)\\
            & DeBERTa  & 68.2~(0.33) & 88.1~(0.15) & 49.7~(0.72) & 54.7~(0.28) & 76.8~(0.42) & 34.0~(0.44)\\
        \midrule
       \multirow{4}{*}{\rotatebox[origin=c]{90}{Bottom-up}} 
            & BERT     & 61.5~(1.32) & 84.9~(1.26) & 39.7~(1.58) & 48.4~(0.12) & 71.4~(0.54) & 26.7~(0.46)\\
            & SpanBERT &67.1~(0.07) & 87.5~(1.16) & 48.2~(1.05) & 53.5~(0.49) & 75.5~(0.30) & 32.8~(0.89)\\
            & RoBERTa  &67.1~(0.25) & 87.2~(0.08) & 48.3~(0.54) & 54.8~(0.28) & 76.2~(0.45) & 34.7~(0.87)\\
            & DeBERTa  &68.1~(0.75) & 88.0~(0.39) & 49.6~(1.14) & 54.4~(0.51) & 76.4~(0.36) & 33.7~(0.68)\\
        \bottomrule
    \end{tabular}
    \caption{Oracle performance considering $k$-best candidates and gold skeleton trees.}
     \label{tab:result_dep_rst}
    \end{table*}


==> contents/tables/dep_rstdtLi14.tex <==
\renewcommand{\arraystretch}{0.85}
\begin{table*}[t]
    \centering
    \small
    %\begin{tabular}{llPPPPPP}
    \begin{tabular}{llcccccc}
    \toprule
     & \multirow{2}{*}{} & \multicolumn{3}{c}{\textbf{UAS}} & \multicolumn{3}{c}{\textbf{LAS}}\\       
    \cmidrule(lr){3-5}\cmidrule(lr){6-8}
    & & \textbf{All}~$\boldsymbol{(d=*)}$ & $\boldsymbol{d=0}$ & $\boldsymbol{d \ge 1}$ & \textbf{All}~$\boldsymbol{(d=*)}$ & $\boldsymbol{d=0}$ & $\boldsymbol{d \ge 1}$ \\
        \midrule
    \multirow{5}{*}{\rotatebox[origin=c]{90}{Top-down}}
            & BERT     & 68.9~(0.28) & 85.6~(0.59) & 49.4~(0.56) & 51.2~(0.50) & 67.5~(0.80) & 32.0~(0.23)\\
            & RoBERTa  & 74.4~(0.18) & \textbf{90.2}~(0.26) & 56.2~(0.34) & 58.1~(0.46) & 74.0~(0.10) & 39.4~(0.83)\\
            & XLNet    & 73.5~(0.81) & 89.5~(0.69) & 55.1~(1.08) & 58.1~(0.71) & 74.0~(0.56) & 39.4~(1.40)\\
            & SpanBERT & 72.6~(0.59) & 88.7~(0.14) & 54.0~(1.16) & 56.2~(0.53) & 72.1~(0.31) & 37.4~(1.52)\\
            & DeBERTa  & \textbf{74.9}~(0.51) & 90.1~(0.04) & \textbf{57.3}~(1.09) & \textbf{59.2}~(0.62) & \textbf{75.0}~(0.36) & \textbf{40.6}~(0.92)\\
        \midrule
       \multirow{5}{*}{\rotatebox[origin=c]{90}{Bottom-up}} 
            & BERT     &  70.3~(0.52) & 87.7~(1.21) & 50.3~(0.57) & 52.8~(0.57) & 69.0~(0.43) & 33.7~(0.72)\\
            & RoBERTa  & 73.4~(1.01) & 89.1~(0.99) & 55.2~(1.01) & 59.0~(0.47) & 74.4~(0.51) & 40.8~(1.04)\\
            & XLNet    & 74.6~(0.30) & \textbf{90.2}~(0.65) & 56.5~(0.72) & 59.5~(0.40) & \textbf{75.2}~(0.63) & 41.0~(1.17)\\
            & SpanBERT & 74.3~(0.36) & 89.2~(0.63) & 57.1~(1.35) & 57.6~(0.51) & 72.9~(0.23) & 39.6~(1.13)\\
            & DeBERTa  & \textbf{75.6}~(0.72) & 89.7~(0.72) & \textbf{59.3}~(0.87) & \textbf{60.1}~(0.71) & 74.7~(0.73) & \textbf{42.9}~(0.83)\\
        \bottomrule
    \end{tabular}
    \caption{Results for dependency format in terms of unlabeled attachment scores (UAS) and labeled attachment scores (LAS). All, $d=0$, and $d \ge 1$ indicate overall scores, scores for cases where the dependency distance is zero, and scores for cases where it is greater than or equal to one, respectively. The best score 
    %in each metric for both strategies 
    is indicated in \textbf{bold}. Results on Instr-DT are shown in Appendix~\ref{app:dep_instr}.}
     \label{tab:result_dep_rst_Li14}
    \end{table*}














==> contents/tables/std_parseval_doc_vs_span.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{lPPPPPPPP}
    \toprule
    %%%%% HEADER %%%%%
     & \multicolumn{4}{c}{\textbf{Top-down}} & \multicolumn{4}{c}{\textbf{Bottom-up}}\\       
    \cmidrule(lr){2-5}\cmidrule(lr){6-9}
     & \textbf{Span} & \textbf{Nuc.} & \textbf{Rel.} & \textbf{Full} & \textbf{Span} & \textbf{Nuc.} & \textbf{Rel.} & \textbf{Full} \\
    \midrule
        %%%%% MAIN RESULTS %%%%
         Span/Action& 
         79.0~(0.04) & 68.4~(0.11) & 57.5~(0.13) & 55.1~(0.12) &
                    79.0~(0.57) & 68.9~(0.36) & 57.5~(0.69) & 55.2~(0.49) \\
         Document   &
                 77.7~(0.42) & 67.1~(0.50) & 54.8~(0.24) & 52.4~(0.52) &
                 77.2~(0.15) & 66.3~(0.63) & 54.9~(0.22) & 52.7~(0.25)\\
              \bottomrule
    \end{tabular}
    \caption{Comparison between span-based batch and document-based batch on the test dataset of RST-DT (DeBERTa). 
    }
    \label{tab:result_base:spanvsdoc}
\end{table*}

==> contents/tables/std_parseval_kbest.tex <==
\renewcommand{\arraystretch}{0.8}
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{llPPPPPPPP}
    \toprule
     & \multirow{2}{*}{} & \multicolumn{4}{c}{\textbf{RST-DT}} & \multicolumn{4}{c}{\textbf{Instr-DT}}\\       
    \cmidrule(lr){3-6}\cmidrule(lr){7-10}
    & & \textbf{Span} & \textbf{Nuc.} & \textbf{Rel.} & \textbf{Full} & \textbf{Span} & \textbf{Nuc.} & \textbf{Rel.} & \textbf{Full} \\
        \midrule
    \multirow{5}{*}{\rotatebox[origin=c]{90}{Top-down}}
    
            & DeBERTa  & 79.0~(0.04) & 68.4~(0.11) & 57.5~(0.13) & 55.1~(0.12) 
                        & 77.5~(0.26) & 57.3~(0.33) & 49.9~(0.19) & 41.9~(0.32)\\          
            & $k=5$    & 80.1~(0.23) & 69.5~(0.18) & 58.6~(0.07) & 56.1~(0.13) 
                       & 79.9~(0.32) & 60.3~(0.07) & 53.1~(0.64) & 45.0~(0.29)\\    
            & $k=10$    & 80.5~(0.20) & 69.9~(0.11) & 59.0~(0.13) & 56.5~(0.16) 
                         & 80.6~(0.38) & 61.4~(0.38) & 54.1~(0.51) & 46.0~(0.19)\\
            & $k=20$    & 80.9~(0.21) & 70.4~(0.14) & 59.5~(0.25) & 57.0~(0.19) 
                        & 81.5~(0.26) & 62.3~(0.51) & 55.0~(0.19) & 46.9~(0.19)\\
            & w/ gold trees & 100~(0.00) & 86.4~(0.11) & 72.1~(0.14) & 68.1~(0.18)
                    & 100~(0.00) & 77.2~(0.69) & 70.4~(0.45) & 59.7~(0.36)\\
        \midrule
       \multirow{5}{*}{\rotatebox[origin=c]{90}{Bottom-up}} 
        & DeBERTa   & 79.0~(0.57) & 68.9~(0.36) & 57.5~(0.69) & 55.2~(0.49)
                    & 75.9~(1.27) & 58.7~(1.07) & 50.0~(1.38) & 43.3~(1.32)\\
        & $k=5$     & 79.7~(0.54) & 69.7~(0.34) & 58.5~(0.62) & 56.2~(0.39)
                    & 78.0~(1.00) & 61.4~(1.07) & 52.4~(1.01) & 45.7~(1.28)\\                    
        & $k=10$    & 80.1~(0.51) & 70.1~(0.30) & 58.9~(0.70) & 56.6~(0.49)
                     & 78.9~(1.46) & 62.6~(1.74) & 53.5~(1.44) & 46.9~(1.74)\\
        & $k=20$    & 80.6~(0.50) & 70.6~(0.24) & 59.5~(0.83) & 57.1~(0.63)
                     & 79.4~(1.36) & 63.2~(1.39) & 54.5~(1.01) & 47.8~(1.36)\\            
        & w/ gold trees & 100~(0.00) & 86.1~(0.27) & 71.7~(0.11) & 67.4~(0.27)
                     & 100~(0.00) & 79.5~(0.69) & 69.6~(0.88) & 60.5~(0.85)\\     
        \bottomrule
    \end{tabular}
    \caption{Oracle performance considering $k$-best candidates and gold skeleton trees.}
     \label{tab:result_kbest}
    \end{table*}



==> contents/tables/std_parseval_large_h_concat.tex <==
\renewcommand{\arraystretch}{0.95}
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{llPPPPPPPP}
    \toprule
     & \multirow{2}{*}{ } & \multicolumn{4}{c}{\textbf{RST-DT}} & \multicolumn{4}{c}{\textbf{Instr-DT}}\\       
    \cmidrule(lr){3-6}\cmidrule(lr){7-10}
    & & \textbf{Span} & \textbf{Nuc.} & \textbf{Rel.} & \textbf{Full} & \textbf{Span} & \textbf{Nuc.} & \textbf{Rel.} & \textbf{Full} \\
        \midrule
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Top-down}}
            & DeBERTa   & 79.0~(0.04) & 68.4~(0.11) & 57.5~(0.13) & 55.1~(0.12)
                        & 77.5~(0.26) & 57.3~(0.33) & 49.9~(0.19) & 41.9~(0.32)\\
            & ~~+CWA      & 80.2~(0.09)& 69.9~(0.22)& 58.3~(0.36) &56.2~(0.39)
                        & 77.8~(0.26)&57.3~(0.14)& 49.9~(0.14)	& 42.0~(0.07)\\
            & ~~w/ \texttt{large} & 80.1~(0.09)&69.7~(0.31)&58.5~(0.28)&56.3~(0.15)
                       & 79.4~(1.36)&62.2~(1.53)&53.3~(0.88)&46.9~(0.50)\\
            & ~~both     & 81.0~(0.22)	& 71.2~(0.56)&60.5~(0.26)&58.3~(0.32)
                       & 79.8~(0.47)&62.6~(0.52)&53.8~(0.59)&47.5~(0.33)\\
        \midrule
       \multirow{4}{*}{\rotatebox[origin=c]{90}{Bottom-up}} 
        & DeBERTa   & 79.0~(0.57) & 68.9~(0.36) & 57.5~(0.69) & 55.2~(0.49)
                        & 75.9~(1.27) & 58.7~(1.07) & 50.0~(1.38) & 43.3~(1.32)\\
        &~~+CWA     & 79.3~(0.30)&	69.6~(0.31)&	58.3~(0.56)&	56.1~(0.53)
                    & 76.0~(0.91)&	59.0~(0.22)&	49.5~(0.87)&43.0~(0.57)\\
        &~~ w/ \texttt{large} & 79.3~(0.98)&	69.1~(0.94)&	58.4~(0.93)&56.0~(0.67)
                    & 78.9~(0.36)&	63.0~(1.24)&	54.7~(0.92)&48.0~(1.19)\\
        &~~both     &80.0~(0.28)&	70.4~(0.16)&	60.0~(0.29)&57.7~(0.35)
                    &79.2~(0.29)	&62.7~(0.47)	& 55.2~(0.19)&	47.9~(0.25)\\
        \bottomrule
    \end{tabular}
    \caption{Results with checkpoint weight averaging (CWA) and the \texttt{large} language model.}
     \label{tab:result_large:horizontal_concat}
    \end{table*}



==> contents/tables/std_parseval_v1_versus_v3.tex <==
\renewcommand{\arraystretch}{1.0}
\begin{table*}[t]
    \centering
    \small
    %\begin{tabular}{llcccccccc}
    \begin{tabular}{lPPPPPPPP}
    \toprule
    %%%%% HEADER %%%%%
     & \multicolumn{4}{c}{\textbf{Three-stage}} & \multicolumn{4}{c}{\textbf{Two-stage}}\\       
    \cmidrule(lr){2-5}\cmidrule(lr){6-9}
     & \textbf{Span} & \textbf{Nuc.} & \textbf{Rel.} & \textbf{Full} & \textbf{Span} & \textbf{Nuc.} & \textbf{Rel.} & \textbf{Full} \\
    \midrule
        %%%%% MAIN RESULTS %%%%
         BERT      & 
                    72.4~(0.65) & 61.1~(0.78) & 51.5~(0.63) & 49.4~(0.29) &
                    72.4~(0.53) & 61.1~(0.71) & 50.7~(0.48) & 48.6~(0.58)\\
         RoBERTa   &
                    76.8~(0.22) & 66.4~(0.64) & 56.7~(0.42) & 54.7~(0.63) &
                    76.1~(0.43) & 65.9~(0.17) & 55.7~(0.18) & 53.6~(0.21)\\    
         XLNet     & 
                    77.0~(0.26) & 66.7~(0.42) &57.5~(0.23) & 55.5~(0.10) &
                    77.6~(0.28) & 67.3~(0.16) &56.8~(0.40) & 54.5~(0.43)\\
         SpanBERT  & 
                    76.2~(0.36) &65.7~(0.12) & 55.6~(0.37) & 53.4~(0.20) &
                    75.6~(0.42) &65.2~(0.41) &55.0~(0.28) & 52.9(0.19)\\
         DeBERTa   & 
                    78.4~(0.23) &68.6~(0.62) & 58.4~(0.63) & 56.1~(0.58) &
                    77.2~(0.56) &67.4~(0.29) &57.6~(0.15) &55.4~(0.23) \\
        \bottomrule
    \end{tabular}
    \caption{Results of two- and three-stage bottom-up parsers on the development dataset in RST-DT.}
    \label{tab:result_base:v1vsv3}
\end{table*}
